Analysis of a contention-based approach over 5G NR for Federated Learning in an Industrial Internet of Things scenario

The growing interest in new applications involving co-located heterogeneous requirements, such as the Industrial Internet of Things (IIoT) paradigm, poses unprecedented challenges to the uplink wireless transmissions. Dedicated scheduling has been the fundamental approach used by mobile radio systems for uplink transmissions, where the network assigns contention-free resources to users based on buffer-related information. The usage of contention-based transmissions was discussed by the 3rd Generation Partnership Project (3GPP) as an alternative approach for reducing the uplink latency characterizing dedicated scheduling. Nevertheless, the contention-based approach was not considered for standardization in LTE due to limited performance gains. However, 5G NR introduced a different radio frame which could change the performance achievable with a contention-based framework, although this has not yet been evaluated. This paper aims to fill this gap. We present a contention-based design introduced for uplink transmissions in a 5G NR IIoT scenario. We provide an up-to-date analysis via near-product 3GPP-compliant network simulations of the achievable application-level performance with simultaneous Ultra-Reliable Low Latency Communications (URLLC) and Federated Learning (FL) traffic, where the contention-based scheme is applied to the FL traffic. The investigation also involves two separate mechanisms for handling retransmissions of lost or collided transmissions. Numerical results show that, under some conditions, the proposed contention-based design provides benefits over dedicated scheduling when considering FL upload/download times, and does not significantly degrade the performance of URLLC.

==> CB_5G_NR_PUSCH_IIoT_Arxiv/acronyms.tex <==
\newacronym{3gpp}{3GPP}{3rd Generation Partnership Project}
\newacronym{adc}{ADC}{Analog to Digital Converter}
\newacronym{5g}{5G}{5th generation}
\newacronym{6g}{6G}{6th generation}
\newacronym{aimd}{AIMD}{Additive Increase Multiplicative Decrease}
\newacronym{amc}{AMC}{Adaptive Modulation and Coding}
\newacronym{aqm}{AQM}{Active Queue Management}
\newacronym{awgn}{AWGN}{Additive White Gaussian Noise}
\newacronym{balia}{BALIA}{Balanced Link Adaptation}
\newacronym{bdp}{BDP}{Bandwidth-Delay Product}
\newacronym{qos}{QoS}{Quality of Service}
\newacronym{pqos}{PQoS}{predictive quality of service}
\newacronym{bf}{BF}{Beamforming}
\newacronym{cc}{CC}{Congestion Control}
\newacronym{cdf}{CDF}{Cumulative Distribution Function}
\newacronym{cn}{CN}{Core Network}
\newacronym{cqi}{CQI}{Channel Quality Information}
\newacronym{cp}{CP}{Control Plane}
\newacronym{csirs}{CSI-RS}{Channel State Information - Reference Signal}
\newacronym{dc}{DC}{Dual Connectivity}
\newacronym{dce}{DCE}{Direct Code Execution}
\newacronym{dci}{DCI}{Downlink Control Information}
\newacronym{dl}{DL}{downlink}
\newacronym{dmr}{DMR}{Deadline Miss Ratio}
\newacronym{dmrs}{DMRS}{DeModulation Reference Signal}
\newacronym{e2e}{E2E}{end-to-end}
\newacronym{ecn}{ECN}{Explicit Congestion Notification}
\newacronym{edf}{EDF}{Earliest Deadline First}
\newacronym{enb}{eNB}{evolved Node Base}
\newacronym{epc}{EPC}{Evolved Packet Core}
\newacronym{es}{ES}{Edge Server}
\newacronym{fdma}{FDMA}{Frequency Division Multiple Access}
\newacronym{fdd}{FDD}{Frequency Division Duplexing}
\newacronym[firstplural=Radio Access Technologies (RATs)]{rat}{RAT}{Radio Access Technology}
\newacronym{fs}{FS}{Fast Switching}
\newacronym{ftp}{FTP}{File Transfer Protocol}
\newacronym{gnb}{gNB}{Next Generation Node Base}
\newacronym{harq}{HARQ}{Hybrid Automatic Repeat reQuest}
\newacronym{hetnet}{HetNet}{Heterogeneous Network}
\newacronym{hh}{HH}{Hard Handover}
\newacronym{hol}{HOL}{Head-of-Line}
\newacronym{ia}{IA}{Initial Access}
\newacronym{ieee}{IEEE}{Institute of Electrical and Electronics Engineers}
\newacronym{imt}{IMT}{International Mobile Telecommunication}
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{ldpc}{LDPC}{Low-Density Parity Check}
\newacronym{los}{LOS}{line-of-sight}
\newacronym{lte}{LTE}{Long Term Evolution}
\newacronym{m2m}{M2M}{Machine to Machine}
\newacronym{ml}{ML}{Machine Learning}
\newacronym{mac}{MAC}{Medium Access Control}
\newacronym{mc}{MC}{Multi-Connectivity}
\newacronym{mcs}{MCS}{Modulation and Coding Scheme}
\newacronym{mec}{MEC}{Mobile Edge Cloud}
\newacronym{mi}{MI}{Mutual Information}
\newacronym{mimo}{MIMO}{Multiple Input Multiple Output}
\newacronym{mmwave}{mmWave}{millimeter wave}
\newacronym{mptcp}{MPTCP}{Multipath TCP}
\newacronym{mr}{MR}{Maximum Rate}
\newacronym{mss}{MSS}{Maximum Segment Size}
\newacronym{mtd}{MTD}{Machine-Type Device}
\newacronym{mtu}{MTU}{Maximum Transmission Unit}
\newacronym{nfv}{NFV}{Network Function Virtualization}
\newacronym{nlos}{NLOS}{non-line-of-sight}
\newacronym{nlosv}{NLOSv}{Vehicle Non-Line-of-Sight}
\newacronym{ofdm}{OFDM}{Orthogonal Frequency Division Multiplexing}
\newacronym{pdcch}{PDCCH}{Physical Downlink Control Channel}
\newacronym{pdcp}{PDCP}{Packet Data Convergence Protocol}
\newacronym{pdsch}{PDSCH}{Physical Downlink Shared Channel}
\newacronym{pdu}{PDU}{Protocol Data Unit}
\newacronym{pf}{PF}{Proportional Fair}
\newacronym{pgw}{PGW}{Packet Gateway}
\newacronym{phy}{PHY}{Physical}
\newacronym{pbch}{PBCH}{Physical Broadcast Channel}
\newacronym[plural=\gls{mme}s,firstplural=Mobility Management Entities (MMEs)]{mme}{MME}{Mobility Management Entity}
\newacronym{prb}{PRB}{Physical Resource Block}
\newacronym{pss}{PSS}{Primary Synchronization Signal}
\newacronym{pscch}{PSCCH}{Physical Sidelink Control Channel}
\newacronym{pucch}{PUCCH}{Physical Uplink Control Channel}
\newacronym{pusch}{PUSCH}{Physical Uplink Shared Channel}
\newacronym{rach}{RACH}{Random Access Channel}
\newacronym{ran}{RAN}{Radio Access Network}
\newacronym{red}{RED}{Random Early Detection}
\newacronym{rf}{RF}{radio frequency}
\newacronym{rlc}{RLC}{Radio Link Control}
\newacronym{rlf}{RLF}{Radio Link Failure}
\newacronym{rrc}{RRC}{Radio Resource Control}
\newacronym{rrm}{RRM}{Radio Resource Management}
\newacronym{rr}{RR}{Round Robin}
\newacronym{rs}{RS}{Remote Server}
\newacronym{rsrp}{RSRP}{Reference Signal Received Power}
\newacronym{rss}{RSS}{Received Signal Strength}
\newacronym{rtt}{RTT}{Round Trip Time}
\newacronym{rw}{RW}{Receive Window}
\newacronym{rx}{RX}{Receiver}
\newacronym{sa}{SA}{standalone}
\newacronym{sack}{SACK}{Selective Acknowledgment}
\newacronym{sap}{SAP}{Service Access Point}
\newacronym{sc}{SC}{Single Carrier}
\newacronym{sch}{SCH}{Secondary Cell Handover}
\newacronym{scoot}{SCOOT}{Split Cycle Offset Optimization Technique}
\newacronym{sdma}{SDMA}{Spatial Division Multiple Access}
\newacronym{sinr}{SINR}{Signal to Interference plus Noise Ratio}
\newacronym{sl}{SL}{Sidelink}
\newacronym{sm}{SM}{Saturation Mode}
\newacronym{snr}{SNR}{Signal-to-Noise-Ratio}
\newacronym{son}{SON}{Self-Organizing Network}
\newacronym{ss}{SS}{Synchronization Signal}
\newacronym{srs}{SRS}{Sounding Reference Signal}
\newacronym{sss}{SSS}{Secondary Synchronization Signal}
\newacronym{tb}{TB}{Transport Block}
\newacronym{tcp}{TCP}{Transmission Control Protocol}
\newacronym{tdd}{TDD}{Time Division Duplexing}
\newacronym{tdma}{TDMA}{Time Division Multiple Access}
\newacronym{tfl}{TfL}{Transport for London}
\newacronym{tm}{TM}{Transparent Mode}
\newacronym{trp}{TRP}{Transmitter Receiver Pair}
\newacronym{tti}{TTI}{Transmission Time Interval}
\newacronym{ttt}{TTT}{Time-to-Trigger}
\newacronym{tx}{TX}{Transmitter}
\newacronym{ue}{UE}{User Equipment}
\newacronym{ul}{UL}{uplink}
\newacronym{uml}{UML}{Unified Modeling Language}
\newacronym{um}{UM}{Unacknowledged Mode}
\newacronym{utc}{UTC}{Urban Traffic Control}
\newacronym{vm}{VM}{Virtual Machine}
\newacronym{rsrq}{RSRQ}{Reference Signal Received Quality}
\newacronym{rssi}{RSSI}{Received Signal Strength Indicator}
\newacronym{crs}{CRS}{Cell Reference Signal}
\newacronym{nsa}{NSA}{Non Stand Alone}
\newacronym{mrdc}{MR-DC}{Multi \gls{rat} \gls{dc}}
\newacronym{endc}{EN-DC}{E-UTRAN-\gls{nr} \gls{dc}}
\newacronym{5gc}{5GC}{5G Core}
\newacronym{si}{SI}{Study Item}
\newacronym{iab}{IAB}{Integrated Access and Backhaul}
\newacronym{wf}{WF}{Wired-first}
\newacronym{hqf}{HQF}{Highest-quality-first}
\newacronym{pa}{PA}{Position-aware}
\newacronym{mlr}{MLR}{Maximum-local-rate}
\newacronym{wbf}{WBF}{Wired Bias Function}
\newacronym{mib}{MIB}{Master Information Block}
\newacronym{sib}{SIB}{Secondary Information Block}
\newacronym{rnti}{RNTI}{Radio Network Temporary Identifier}
\newacronym{dft}{DFT}{Discrete Fourier Transform}
\newacronym{kpi}{KPI}{Key Performance Indicator}
\newacronym{ppp}{PPP}{Poisson Point Process}
\newacronym{v2v}{V2V}{Vehicle-to-Vehicle}
\newacronym{wave}{WAVE}{Wireless Access in Vehicular Environments}
\newacronym{udp}{UDP}{User Datagram Protocol}
\newacronym{upa}{UPA}{Uniform Planar Array}
\newacronym{fec}{FEC}{Forward Error Correction}
\newacronym{v2x}{V2X}{Vehicle-To-Everything}
\newacronym{psfch}{PSFCH}{Physical Sidelink Feedback Channel}
\newacronym{pssch}{PSSCH}{Physical Sidelink Shared Channel}
\newacronym{csma}{CSMA}{Carrier Sense Multiple Access}
\newacronym{v2n}{V2N}{Vehicle-to-Network}
\newacronym{wlan}{WLAN}{Wireless Local Area Network}
\newacronym{cav}{CAV}{Connected and Autonomous Vehicle}
\newacronym{v2i}{V2I}{Vehicle-to-Infrastructure}
\newacronym{d2d}{D2D}{Device-to-Device}
\newacronym{c-its}{C-ITS}{Connected Intelligent Transportation System}
\newacronym{fr2}{FR2}{Frequency Range 2}
\newacronym{fr1}{FR1}{Frequency Range 1}
\newacronym{bs}{BS}{Base Station}
\newacronym{sdu}{SDU}{Service Data Unit}
\newacronym{csi}{CSI}{Channel State Information}
\newacronym{scs}{SCS}{Subcarrier Spacing}
\newacronym{sumo}{SUMO}{Simulation of Urban MObility}
\newacronym{prr}{PRR}{Packet Reception Ratio}
\newacronym{edca}{EDCA}{Enhanced Distribution Channel Access}
\newacronym{sdap}{SDAP}{Service Data Adaptation Protocol}
\newacronym{iiot}{IIoT}{Industrial Internet of Things}
\newacronym{agv}{AGV}{Automated Guided Vehicle}
\newacronym{cm}{C/M}{Controller/Master}
\newacronym{soa}{SoA}{State-of-the-Art}
\newacronym{snpn}{SNPN}{Standalone Non-Public Network}
\newacronym{pninpn}{PNI-NPN}{Public Network Interface Non-Public Network}
\newacronym{urllc}{URLLC}{Ultra-Reliable Low-Latency Communication}
\newacronym{embb}{eMBB}{enhanced Mobile BroadBand}
\newacronym{ai}{AI}{Artificial Intelligence}
\newacronym{mab}{MAB}{Multi-Armed Bandit}
\newacronym{su}{SU}{Scheduling Unit}
\newacronym{ra}{RA}{Random Agent}
\newacronym{na}{NA}{Neural Agent}
\newacronym{ucba}{UCB-A}{UCB Agent}
\newacronym{tsa}{TS-A}{Thompson Sampling Agent}
\newacronym{ucb}{UCB}{Upper Confidence Bound}
\newacronym{ts}{TS}{Thompson Sampling}
\newacronym{inf}{InF}{Indoor Factory}
\newacronym{infsl}{InF-SL}{Indoor Factory - Sparse Clutter, Low BS}
\newacronym{infdl}{InF-DL}{Indoor Factory - Dense Clutter, Low BS}
\newacronym{infsh}{InF-SH}{Indoor Factory - Sparse Clutter, High BS}
\newacronym{infdh}{InF-DH}{Indoor Factory - Dense Clutter, High BS}
\newacronym{us}{US}{Uplink Scheduler}
\newacronym{nn}{NN}{Neural Network}
\newacronym{das}{DAS}{Distributed Antenna System}
\newacronym{rb}{RB}{Resource Block}
\newacronym{rl}{RL}{Reinforcement Learning}
\newacronym{uav}{UAV}{Unmanned Aerial Vehicle}
\newacronym{5gacia}{5G-ACIA}{5G Alliance for Connected Industries and Automation}
\newacronym{fl}{FL}{Federated Learning}
\newacronym{ack}{ACK}{Acknowledgment} 
\newacronym{dnn}{DNN}{Deep Neural Network}
\newacronym{sr}{SR}{Scheduling Request}
\newacronym{bsr}{BSR}{Buffer Status Report}
\newacronym{nr}{NR}{New Radio}
\newacronym{cb}{CB}{Contention-Based}
\newacronym{cf}{CF}{Contention-Free}
\newacronym{ce}{CE}{Control Element}
\newacronym{sps}{SPS}{Semi-Persistent Scheduling}
\newacronym{ds}{DS}{Dynamic Scheduling}
\newacronym{xr}{XR}{Extended Reality}
\newacronym{ofdma}{OFDMA}{Orthogonal Frequency Division Multiple Access}
\newacronym{cdma}{CDMA}{Code Division Multiple Access}
\newacronym{noma}{NOMA}{Non-Orthogonal Multiple Access}
\newacronym{ibi}{IBI}{Instantaneous Buffer Information}
\newacronym{am}{AM}{Acknowledge Mode}

==> CB_5G_NR_PUSCH_IIoT_Arxiv/ieeeaccess_suggestions.tex <==
% These instructions give you guidelines for preparing papers for 
% IEEE Access. Use this document as a template if you are 
% using \LaTeX. Otherwise, use this document as an 
% instruction set. The electronic file of your paper will be formatted further 
% at IEEE. Paper titles should be written in uppercase and lowercase letters, 
% not all uppercase. Avoid writing long formulas with subscripts in the title; 
% short formulas that identify the elements are fine (e.g., "Nd--Fe--B"). Do 
% not write ``(Invited)'' in the title. Full names of authors are preferred in 
% the author field, but are not required. Put a space between authors' 
% initials. The abstract must be a concise yet comprehensive reflection of 
% what is in your article. In particular, the abstract must be self-contained, 
% without abbreviations, footnotes, or references. It should be a microcosm of 
% the full article. The abstract must be between 150--250 words. Be sure that 
% you adhere to these limits; otherwise, you will need to edit your abstract 
% accordingly. The abstract must be written as one paragraph, and should not 
% contain displayed mathematical equations or tabular material. The abstract 
% should include three or four different keywords or phrases, as this will 
% help readers to find it. It is important to avoid over-repetition of such 
% phrases as this can result in a page being rejected by search engines. 
% Ensure that your abstract reads well and is grammatically correct.

% Enter key words or phrases in alphabetical 
% order, separated by commas. For a list of suggested keywords, send a blank 
% e-mail to keywords@ieee.org or visit \underline
% {http://www.ieee.org/organizations/pubs/ani\_prod/keywrd98.txt}

% Use one space after periods and colons. Hyphenate complex modifiers: 
% ``zero-field-cooled magnetization.'' Avoid dangling participles, such as, 
% ``Using \eqref{eq}, the potential was calculated.'' [It is not clear who or what 
% used \eqref{eq}.] Write instead, ``The potential was calculated by using \eqref{eq},'' or 
% ``Using \eqref{eq}, we calculated the potential.''

% Use a zero before decimal points: ``0.25,'' not ``.25.'' Use 
% ``cm$^{3}$,'' not ``cc.'' Indicate sample dimensions as ``0.1 cm 
% $\times $ 0.2 cm,'' not ``0.1 $\times $ 0.2 cm$^{2}$.'' The 
% abbreviation for ``seconds'' is ``s,'' not ``sec.'' Use 
% ``Wb/m$^{2}$'' or ``webers per square meter,'' not 
% ``webers/m$^{2}$.'' When expressing a range of values, write ``7 to 
% 9'' or ``7--9,'' not ``7$\sim $9.''

% A parenthetical statement at the end of a sentence is punctuated outside of 
% the closing parenthesis (like this). (A parenthetical sentence is punctuated 
% within the parentheses.) In American English, periods and commas are within 
% quotation marks, like ``this period.'' Other punctuation is ``outside''! 
% Avoid contractions; for example, write ``do not'' instead of ``don't.'' The 
% serial comma is preferred: ``A, B, and C'' instead of ``A, B and C.''

% If you wish, you may write in the first person singular or plural and use 
% the active voice (``I observed that $\ldots$'' or ``We observed that $\ldots$'' 
% instead of ``It was observed that $\ldots$''). Remember to check spelling. If 
% your native language is not English, please get a native English-speaking 
% colleague to carefully proofread your paper.

% Try not to use too many typefaces in the same article. You're writing
% scholarly papers, not ransom notes. Also please remember that MathJax
% can't handle really weird typefaces.

% Number equations consecutively with equation numbers in parentheses flush 
% with the right margin, as in \eqref{eq}. To make your equations more 
% compact, you may use the solidus (~/~), the exp function, or appropriate 
% exponents. Use parentheses to avoid ambiguities in denominators. Punctuate 
% equations when they are part of a sentence, as in
% \begin{equation}E=mc^2.\label{eq}\end{equation}

% Be sure that the symbols in your equation have been defined before the 
% equation appears or immediately following. Italicize symbols ($T$ might refer 
% to temperature, but T is the unit tesla). Refer to ``\eqref{eq},'' not ``Eq. \eqref{eq}'' 
% or ``equation \eqref{eq},'' except at the beginning of a sentence: ``Equation \eqref{eq} 
% is $\ldots$ .''

% Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
% of ``hard'' references (e.g., \verb|(1)|). That will make it possible
% to combine sections, add equations, or change the order of figures or
% citations without having to go through the file line by line.

% Please don't use the \verb|{eqnarray}| equation environment. Use
% \verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
% environment leaves unsightly spaces around relation symbols.
% Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
% will not stop equation numbers inside \verb|{array}| (there won't be
% any anyway) and it might stop a wanted equation number in the
% surrounding equation.

% Please note that the \verb|{subequations}| environment in {\LaTeX}
% will increment the main equation counter even when there are no
% equation numbers displayed. If you forget that, you might write an
% article in which the equation numbers skip from (17) to (20), causing
% the copy editors to wonder if you've discovered a new method of
% counting.

% {\BibTeX} does not work by magic. It doesn't get the bibliographic
% data from thin air but from .bib files. If you use {\BibTeX} to produce a
% bibliography you must send the .bib files. 

% {\LaTeX} can't read your mind. If you assign the same label to a
% subsubsection and a table, you might find that Table I has been cross
% referenced as Table IV-B3. 

% {\LaTeX} does not have precognitive abilities. If you put a
% \verb|\label| command before the command that updates the counter it's
% supposed to be using, the label will pick up the last counter to be
% cross referenced instead. In particular, a \verb|\label| command
% should not go before the caption of a figure or a table.

% Use either SI (MKS) or CGS as primary units. (SI units are strongly 
% encouraged.) English units may be used as secondary units (in parentheses). 
% This applies to papers in data storage. For example, write ``15 
% Gb/cm$^{2}$ (100 Gb/in$^{2})$.'' An exception is when 
% English units are used as identifiers in trade, such as ``3\textonehalf-in 
% disk drive.'' Avoid combining SI and CGS units, such as current in amperes 
% and magnetic field in oersteds. This often leads to confusion because 
% equations do not balance dimensionally. If you must use mixed units, clearly 
% state the units for each quantity in an equation.

% The SI unit for magnetic field strength $H$ is A/m. However, if you wish to use 
% units of T, either refer to magnetic flux density $B$ or magnetic field 
% strength symbolized as $\mu _{0}H$. Use the center dot to separate 
% compound units, e.g., ``A$\cdot $m$^{2}$.''

% The word ``data'' is plural, not singular. The subscript for the 
% permeability of vacuum $\mu _{0}$ is zero, not a lowercase letter 
% ``o.'' The term for residual magnetization is ``remanence''; the adjective 
% is ``remanent''; do not write ``remnance'' or ``remnant.'' Use the word 
% ``micrometer'' instead of ``micron.'' A graph within a graph is an 
% ``inset,'' not an ``insert.'' The word ``alternatively'' is preferred to the 
% word ``alternately'' (unless you really mean something that alternates). Use 
% the word ``whereas'' instead of ``while'' (unless you are referring to 
% simultaneous events). Do not use the word ``essentially'' to mean 
% ``approximately'' or ``effectively.'' Do not use the word ``issue'' as a 
% euphemism for ``problem.'' When compositions are not specified, separate 
% chemical symbols by en-dashes; for example, ``NiMn'' indicates the 
% intermetallic compound Ni$_{0.5}$Mn$_{0.5}$ whereas 
% ``Ni--Mn'' indicates an alloy of some composition 
% Ni$_{x}$Mn$_{1-x}$.

% \Figure[t!](topskip=0pt, botskip=0pt, midskip=0pt)[width=3.25in]{figures/scenario.png}
% {Caption. \label{fig:scenario}}

% Be aware of the different meanings of the homophones ``affect'' (usually a 
% verb) and ``effect'' (usually a noun), ``complement'' and ``compliment,'' 
% ``discreet'' and ``discrete,'' ``principal'' (e.g., ``principal 
% investigator'') and ``principle'' (e.g., ``principle of measurement''). Do 
% not confuse ``imply'' and ``infer.'' 

% Prefixes such as ``non,'' ``sub,'' ``micro,'' ``multi,'' and ``ultra'' are 
% not independent words; they should be joined to the words they modify, 
% usually without a hyphen. There is no period after the ``et'' in the Latin 
% abbreviation ``\emph{et al.}'' (it is also italicized). The abbreviation ``i.e.,'' means 
% ``that is,'' and the abbreviation ``e.g.,'' means ``for example'' (these 
% abbreviations are not italicized).

% A general IEEE styleguide is available at \underline{http://www.ieee.org/}\break\underline{authortools}.

% \subsection{Types of Graphics}
% The following list outlines the different types of graphics published in 
% IEEE journals. They are categorized based on their construction, and use of 
% color/shades of gray:

% \subsubsection{Color/Grayscale figures}
% {Figures that are meant to appear in color, or shades of black/gray. Such 
% figures may include photographs, illustrations, multicolor graphs, and 
% flowcharts.}

% \subsubsection{Line Art figures}
% {Figures that are composed of only black lines and shapes. These figures 
% should have no shades or half-tones of gray, only black and white.}

% \subsubsection{Author photos}
% {Head and shoulders shots of authors that appear at the end of our papers. }

% \subsubsection{Tables}
% {Data charts which are typically black and white, but sometimes include 
% color.}

% \begin{table}
% \caption{Units for Magnetic Properties}
% \label{table}
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{|p{25pt}|p{75pt}|p{115pt}|}
% \hline
% Symbol& 
% Quantity& 
% Conversion from Gaussian and \par CGS EMU to SI $^{\mathrm{a}}$ \\
% \hline
% $\Phi $& 
% magnetic flux& 
% 1 Mx $\to  10^{-8}$ Wb $= 10^{-8}$ V$\cdot $s \\
% $B$& 
% magnetic flux density, \par magnetic induction& 
% 1 G $\to  10^{-4}$ T $= 10^{-4}$ Wb/m$^{2}$ \\
% $H$& 
% magnetic field strength& 
% 1 Oe $\to  10^{3}/(4\pi )$ A/m \\
% $m$& 
% magnetic moment& 
% 1 erg/G $=$ 1 emu \par $\to 10^{-3}$ A$\cdot $m$^{2} = 10^{-3}$ J/T \\
% $M$& 
% magnetization& 
% 1 erg/(G$\cdot $cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 10^{3}$ A/m \\
% 4$\pi M$& 
% magnetization& 
% 1 G $\to  10^{3}/(4\pi )$ A/m \\
% $\sigma $& 
% specific magnetization& 
% 1 erg/(G$\cdot $g) $=$ 1 emu/g $\to $ 1 A$\cdot $m$^{2}$/kg \\
% $j$& 
% magnetic dipole \par moment& 
% 1 erg/G $=$ 1 emu \par $\to 4\pi \times  10^{-10}$ Wb$\cdot $m \\
% $J$& 
% magnetic polarization& 
% 1 erg/(G$\cdot $cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 4\pi \times  10^{-4}$ T \\
% $\chi , \kappa $& 
% susceptibility& 
% 1 $\to  4\pi $ \\
% $\chi_{\rho }$& 
% mass susceptibility& 
% 1 cm$^{3}$/g $\to  4\pi \times  10^{-3}$ m$^{3}$/kg \\
% $\mu $& 
% permeability& 
% 1 $\to  4\pi \times  10^{-7}$ H/m \par $= 4\pi \times  10^{-7}$ Wb/(A$\cdot $m) \\
% $\mu_{r}$& 
% relative permeability& 
% $\mu \to \mu_{r}$ \\
% $w, W$& 
% energy density& 
% 1 erg/cm$^{3} \to  10^{-1}$ J/m$^{3}$ \\
% $N, D$& 
% demagnetizing factor& 
% 1 $\to  1/(4\pi )$ \\
% \hline
% \multicolumn{3}{p{251pt}}{Vertical lines are optional in tables. Statements that serve as captions for 
% the entire table do not need footnote letters. }\\
% \multicolumn{3}{p{251pt}}{$^{\mathrm{a}}$Gaussian units are the same as cg emu for magnetostatics; Mx 
% $=$ maxwell, G $=$ gauss, Oe $=$ oersted; Wb $=$ weber, V $=$ volt, s $=$ 
% second, T $=$ tesla, m $=$ meter, A $=$ ampere, J $=$ joule, kg $=$ 
% kilogram, H $=$ henry.}
% \end{tabular}
% \label{tab1}
% \end{table}

% \subsection{Multipart figures}
% Figures compiled of more than one sub-figure presented side-by-side, or 
% stacked. If a multipart figure is made up of multiple figure
% types (one part is lineart, and another is grayscale or color) the figure 
% should meet the stricter guidelines.

% \subsection{File Formats For Graphics}\label{formats}
% Format and save your graphics using a suitable graphics processing program 
% that will allow you to create the images as PostScript (PS), Encapsulated 
% PostScript (.EPS), Tagged Image File Format (.TIFF), Portable Document 
% Format (.PDF), Portable Network Graphics (.PNG), or Metapost (.MPS), sizes them, and adjusts 
% the resolution settings. When 
% submitting your final paper, your graphics should all be submitted 
% individually in one of these formats along with the manuscript.

% \subsection{Sizing of Graphics}
% Most charts, graphs, and tables are one column wide (3.5 inches/88 
% millimeters/21 picas) or page wide (7.16 inches/181 millimeters/43 
% picas). The maximum depth a graphic can be is 8.5 inches (216 millimeters/54
% picas). When choosing the depth of a graphic, please allow space for a 
% caption. Figures can be sized between column and page widths if the author 
% chooses, however it is recommended that figures are not sized less than 
% column width unless when necessary. 

% There is currently one publication with column measurements that do not 
% coincide with those listed above. Proceedings of the IEEE has a column 
% measurement of 3.25 inches (82.5 millimeters/19.5 picas). 

% The final printed size of author photographs is exactly
% 1 inch wide by 1.25 inches tall (25.4 millimeters$\,\times\,$31.75 millimeters/6 
% picas$\,\times\,$7.5 picas). Author photos printed in editorials measure 1.59 inches 
% wide by 2 inches tall (40 millimeters$\,\times\,$50 millimeters/9.5 picas$\,\times\,$12 
% picas).

% \subsection{Resolution }
% The proper resolution of your figures will depend on the type of figure it 
% is as defined in the ``Types of Figures'' section. Author photographs, 
% color, and grayscale figures should be at least 300dpi. Line art, including 
% tables should be a minimum of 600dpi.

% \subsection{Vector Art}
% In order to preserve the figures' integrity across multiple computer 
% platforms, we accept files in the following formats: .EPS/.PDF/.PS. All 
% fonts must be embedded or text converted to outlines in order to achieve the 
% best-quality results.

% \subsection{Color Space}
% The term color space refers to the entire sum of colors that can be 
% represented within the said medium. For our purposes, the three main color 
% spaces are Grayscale, RGB (red/green/blue) and CMYK 
% (cyan/magenta/yellow/black). RGB is generally used with on-screen graphics, 
% whereas CMYK is used for printing purposes.

% All color figures should be generated in RGB or CMYK color space. Grayscale 
% images should be submitted in Grayscale color space. Line art may be 
% provided in grayscale OR bitmap colorspace. Note that ``bitmap colorspace'' 
% and ``bitmap file format'' are not the same thing. When bitmap color space 
% is selected, .TIF/.TIFF/.PNG are the recommended file formats.

% \subsection{Accepted Fonts Within Figures}
% When preparing your graphics IEEE suggests that you use of one of the 
% following Open Type fonts: Times New Roman, Helvetica, Arial, Cambria, and 
% Symbol. If you are supplying EPS, PS, or PDF files all fonts must be 
% embedded. Some fonts may only be native to your operating system; without 
% the fonts embedded, parts of the graphic may be distorted or missing.

% A safe option when finalizing your figures is to strip out the fonts before 
% you save the files, creating ``outline'' type. This converts fonts to 
% artwork what will appear uniformly on any screen.

% \subsection{Using Labels Within Figures}

% \subsubsection{Figure Axis labels }
% Figure axis labels are often a source of confusion. Use words rather than 
% symbols. As an example, write the quantity ``Magnetization,'' or 
% ``Magnetization M,'' not just ``M.'' Put units in parentheses. Do not label 
% axes only with units. As in Fig. 1, for example, write ``Magnetization 
% (A/m)'' or ``Magnetization (A$\cdot$m$^{-1}$),'' not just ``A/m.'' Do not label axes with a ratio of quantities and 
% units. For example, write ``Temperature (K),'' not ``Temperature/K.'' 

% Multipliers can be especially confusing. Write ``Magnetization (kA/m)'' or 
% ``Magnetization (10$^{3}$ A/m).'' Do not write ``Magnetization 
% (A/m)$\,\times\,$1000'' because the reader would not know whether the top 
% axis label in Fig. 1 meant 16000 A/m or 0.016 A/m. Figure labels should be 
% legible, approximately 8 to 10 point type.

% \subsubsection{Subfigure Labels in Multipart Figures and Tables}
% Multipart figures should be combined and labeled before final submission. 
% Labels should appear centered below each subfigure in 8 point Times New 
% Roman font in the format of (a) (b) (c). 

% \subsection{Referencing a Figure or Table Within Your Paper}
% When referencing your figures and tables within your paper, use the 
% abbreviation ``Fig.'' even at the beginning of a sentence. Do not abbreviate 
% ``Table.'' Tables should be numbered with Roman Numerals.

% \subsection{Checking Your Figures: The IEEE Graphics Analyzer}
% The IEEE Graphics Analyzer enables authors to pre-screen their graphics for 
% compliance with IEEE Access standards before submission. 
% The online tool, located at
% \underline{http://graphicsqc.ieee.org/}, allows authors to 
% upload their graphics in order to check that each file is the correct file 
% format, resolution, size and colorspace; that no fonts are missing or 
% corrupt; that figures are not compiled in layers or have transparency, and 
% that they are named according to the IEEE Access naming 
% convention. At the end of this automated process, authors are provided with 
% a detailed report on each graphic within the web applet, as well as by 
% email.

% For more information on using the Graphics Analyzer or any other graphics 
% related topic, contact the IEEE Graphics Help Desk by e-mail at 
% graphics@ieee.org.

% \subsection{Submitting Your Graphics}
% Because IEEE will do the final formatting of your paper,
% you do not need to position figures and tables at the top and bottom of each 
% column. In fact, all figures, figure captions, and tables can be placed at 
% the end of your paper. In addition to, or even in lieu of submitting figures 
% within your final manuscript, figures should be submitted individually, 
% separate from the manuscript in one of the file formats listed above in 
% Section \ref{formats}. Place figure captions below the figures; place table titles 
% above the tables. Please do not include captions as part of the figures, or 
% put them in ``text boxes'' linked to the figures. Also, do not place borders 
% around the outside of your figures.

% \subsection{Color Processing/Printing in IEEE Journals}
% All IEEE Transactions, Journals, and Letters allow an author to publish 
% color figures on IEEE Xplore\textregistered\ at no charge, and automatically 
% convert them to grayscale for print versions. In most journals, figures and 
% tables may alternatively be printed in color if an author chooses to do so. 
% Please note that this service comes at an extra expense to the author. If 
% you intend to have print color graphics, include a note with your final 
% paper indicating which figures or tables you would like to be handled that 
% way, and stating that you are willing to pay the additional fee.

% A conclusion section is not required. Although a conclusion may review the 
% main points of the paper, do not replicate the abstract as the conclusion. A 
% conclusion might elaborate on the importance of the work or suggest 
% applications and extensions. 

% Appendixes, if needed, appear before the acknowledgment.

% \section*{Acknowledgment}

% The preferred spelling of the word ``acknowledgment'' in American English is 
% without an ``e'' after the ``g.'' Use the singular heading even if you have 
% many acknowledgments. Avoid expressions such as ``One of us (S.B.A.) would 
% like to thank $\ldots$ .'' Instead, write ``F. A. Author thanks $\ldots$ .'' In most 
% cases, sponsor and financial support acknowledgments are placed in the 
% unnumbered footnote on the first page, not here.

% \section*{References and Footnotes}

% \subsection{References}
% References need not be cited in text. When they are, they appear on the 
% line, in square brackets, inside the punctuation. Multiple references are 
% each numbered with separate brackets. When citing a section in a book, 
% please give the relevant page numbers. In text, refer simply to the 
% reference number. Do not use ``Ref.'' or ``reference'' except at the 
% beginning of a sentence: ``Reference b3 shows $\ldots$ .'' Please do not use 
% automatic endnotes in \emph{Word}, rather, type the reference list at the end of the 
% paper using the ``References'' style. \GC{Added a trial reference \cite{3gpp22874}}.

% Reference numbers are set flush left and form a column of their own, hanging 
% out beyond the body of the reference. The reference numbers are on the line, 
% enclosed in square brackets. In all references, the given name of the author 
% or editor is abbreviated to the initial only and precedes the last name. Use 
% them all; use \emph{et al.} only if names are not given. Use commas around Jr., 
% Sr., and III in names. Abbreviate conference titles. When citing IEEE 
% transactions, provide the issue number, page range, volume number, year, 
% and/or month if available. When referencing a patent, provide the day and 
% the month of issue, or application. References may not include all 
% information; please obtain and include relevant information. Do not combine 
% references. There must be only one reference with each number. If there is a 
% URL included with the print reference, it can be included at the end of the 
% reference. 

% Other than books, capitalize only the first word in a paper title, except 
% for proper nouns and element symbols. For papers published in translation 
% journals, please give the English citation first, followed by the original 
% foreign-language citation See the end of this document for formats and 
% examples of common references. For a complete discussion of references and 
% their formats, see the IEEE style manual at
% \underline{http://www.ieee.org/authortools}.


% \section{Submitting Your Paper for Review}

% \subsection{Final Stage}
% When you submit your final version (after your paper has been accepted), 
% print it in two-column format, including figures and tables. You must also 
% send your final manuscript on a disk, via e-mail, or through a Web 
% manuscript submission system as directed by the society contact. You may use 
% \emph{Zip} for large files, or compress files using \emph{Compress, Pkzip, Stuffit,} or \emph{Gzip.} 

% Also, send a sheet of paper or PDF with complete contact information for all 
% authors. Include full mailing addresses, telephone numbers, fax numbers, and 
% e-mail addresses. This information will be used to send each author a 
% complimentary copy of the journal in which the paper appears. In addition, 
% designate one author as the ``corresponding author.'' This is the author to 
% whom proofs of the paper will be sent. Proofs are sent to the corresponding 
% author only.

% \subsection{Review Stage Using ScholarOne\textregistered\ Manuscripts}
% Contributions to the Transactions, Journals, and Letters may be submitted 
% electronically on IEEE's on-line manuscript submission and peer-review 
% system, ScholarOne\textregistered\ Manuscripts. You can get a listing of the 
% publications that participate in ScholarOne at 
% \underline{http://www.ieee.org/publications\_standards/publications/}\break\underline{authors/authors\_submission.html}.
% First check if you have an existing account. If there is none, please create 
% a new account. After logging in, go to your Author Center and click ``Submit 
% First Draft of a New Manuscript.'' 

% Along with other information, you will be asked to select the subject from a 
% pull-down list. Depending on the journal, there are various steps to the 
% submission process; you must complete all steps for a complete submission. 
% At the end of each step you must click ``Save and Continue''; just uploading 
% the paper is not sufficient. After the last step, you should see a 
% confirmation that the submission is complete. You should also receive an 
% e-mail confirmation. For inquiries regarding the submission of your paper on 
% ScholarOne Manuscripts, please contact oprs-support@ieee.org or call +1 732 
% 465 5861.

% ScholarOne Manuscripts will accept files for review in various formats. 
% Please check the guidelines of the specific journal for which you plan to 
% submit.

% You will be asked to file an electronic copyright form immediately upon 
% completing the submission process (authors are responsible for obtaining any 
% security clearances). Failure to submit the electronic copyright could 
% result in publishing delays later. You will also have the opportunity to 
% designate your article as ``open access'' if you agree to pay the IEEE open 
% access fee. 

% \subsection{Final Stage Using ScholarOne Manuscripts}
% Upon acceptance, you will receive an email with specific instructions 
% regarding the submission of your final files. To avoid any delays in 
% publication, please be sure to follow these instructions. Most journals 
% require that final submissions be uploaded through ScholarOne Manuscripts, 
% although some may still accept final submissions via email. Final 
% submissions should include source files of your accepted manuscript, high 
% quality graphic files, and a formatted pdf file. If you have any questions 
% regarding the final submission process, please contact the administrative 
% contact for the journal. 

% In addition to this, upload a file with complete contact information for all 
% authors. Include full mailing addresses, telephone numbers, fax numbers, and 
% e-mail addresses. Designate the author who submitted the manuscript on 
% ScholarOne Manuscripts as the ``corresponding author.'' This is the only 
% author to whom proofs of the paper will be sent. 

% \subsection{Footnotes}
% Number footnotes separately in superscript numbers.\footnote{It is recommended that footnotes be avoided (except for 
% the unnumbered footnote with the receipt date on the first page). Instead, 
% try to integrate the footnote information into the text.} Place the actual 
% footnote at the bottom of the column in which it is cited; do not put 
% footnotes in the reference list (endnotes). Use letters for table footnotes 
% (see Table \ref{table}).

% \subsection{Copyright Form}
% Authors must submit an electronic IEEE Copyright Form (eCF) upon submitting 
% their final manuscript files. You can access the eCF system through your 
% manuscript submission system or through the Author Gateway. You are 
% responsible for obtaining any necessary approvals and/or security 
% clearances. For additional information on intellectual property rights, 
% visit the IEEE Intellectual Property Rights department web page at 
% \underline{http://www.ieee.org/publications\_standards/publications/}\break\underline{rights/index.html}. 

% \section{IEEE Publishing Policy}
% The general IEEE policy requires that authors should only submit original 
% work that has neither appeared elsewhere for publication, nor is under 
% review for another refereed publication. The submitting author must disclose 
% all prior publication(s) and current submissions when submitting a 
% manuscript. Do not publish ``preliminary'' data or results. The submitting 
% author is responsible for obtaining agreement of all coauthors and any 
% consent required from employers or sponsors before submitting an article. 
% The IEEE Access Department strongly discourages courtesy 
% authorship; it is the obligation of the authors to cite only relevant prior 
% work.

% The IEEE Access Department does not publish conference 
% records or proceedings, but can publish articles related to conferences that 
% have undergone rigorous peer review. Minimally, two reviews are required for 
% every article submitted for peer review.

% \section{Publication Principles}
% The two types of contents of that are published are; 1) peer-reviewed and 2) 
% archival. The Access Department publishes scholarly 
% articles of archival value as well as tutorial expositions and critical 
% reviews of classical subjects and topics of current interest. 

% Authors should consider the following points:

% \begin{enumerate}
% \item Technical papers submitted for publication must advance the state of knowledge and must cite relevant prior work. 
% \item The length of a submitted paper should be commensurate with the importance, or appropriate to the complexity, of the work. For example, an obvious extension of previously published work might not be appropriate for publication or might be adequately treated in just a few pages.
% \item Authors must convince both peer reviewers and the editors of the scientific and technical merit of a paper; the standards of proof are higher when extraordinary or unexpected results are reported. 
% \item Because replication is required for scientific progress, papers submitted for publication must provide sufficient information to allow readers to perform similar experiments or calculations and 
% use the reported results. Although not everything need be disclosed, a paper 
% must contain new, useable, and fully described information. For example, a 
% specimen's chemical composition need not be reported if the main purpose of 
% a paper is to introduce a new measurement technique. Authors should expect 
% to be challenged by reviewers if the results are not supported by adequate 
% data and critical details.
% \item Papers that describe ongoing work or announce the latest technical achievement, which are suitable for presentation at a professional conference, may not be appropriate for publication.
% \end{enumerate}

% \section{Reference Examples}

% \begin{itemize}

% \item \emph{Basic format for books:}\\
% J. K. Author, ``Title of chapter in the book,'' in \emph{Title of His Published Book, x}th ed. City of Publisher, (only U.S. State), Country: Abbrev. of Publisher, year, ch. $x$, sec. $x$, pp. \emph{xxx--xxx.}\\
% See \cite{b1,b2}.

% \item \emph{Basic format for periodicals:}\\
% J. K. Author, ``Name of paper,'' \emph{Abbrev. Title of Periodical}, vol. \emph{x, no}. $x, $pp\emph{. xxx--xxx, }Abbrev. Month, year, DOI. 10.1109.\emph{XXX}.123456.\\
% See \cite{b3}--\cite{b5}.

% \item \emph{Basic format for reports:}\\
% J. K. Author, ``Title of report,'' Abbrev. Name of Co., City of Co., Abbrev. State, Country, Rep. \emph{xxx}, year.\\
% See \cite{b6,b7}.

% \item \emph{Basic format for handbooks:}\\
% \emph{Name of Manual/Handbook, x} ed., Abbrev. Name of Co., City of Co., Abbrev. State, Country, year, pp. \emph{xxx--xxx.}\\
% See \cite{b8,b9}.

% \item \emph{Basic format for books (when available online):}\\
% J. K. Author, ``Title of chapter in the book,'' in \emph{Title of
% Published Book}, $x$th ed. City of Publisher, State, Country: Abbrev.
% of Publisher, year, ch. $x$, sec. $x$, pp. \emph{xxx--xxx}. [Online].
% Available: \underline{http://www.web.com}\\
% See \cite{b10}--\cite{b13}.

% \item \emph{Basic format for journals (when available online):}\\
% J. K. Author, ``Name of paper,'' \emph{Abbrev. Title of Periodical}, vol. $x$, no. $x$, pp. \emph{xxx--xxx}, Abbrev. Month, year. Accessed on: Month, Day, year, DOI: 10.1109.\emph{XXX}.123456, [Online].\\
% See \cite{b14}--\cite{b16}.

% \item \emph{Basic format for papers presented at conferences (when available online): }\\
% J.K. Author. (year, month). Title. presented at abbrev. conference title. [Type of Medium]. Available: site/path/file\\
% See \cite{b17}.

% \item \emph{Basic format for reports and handbooks (when available online):}\\
% J. K. Author. ``Title of report,'' Company. City, State, Country. Rep. no., (optional: vol./issue), Date. [Online] Available: site/path/file\\
% See \cite{b18,b19}.

% \item \emph{Basic format for computer programs and electronic documents (when available online): }\\
% Legislative body. Number of Congress, Session. (year, month day). \emph{Number of bill or resolution}, \emph{Title}. [Type of medium]. Available: site/path/file\\
% \textbf{\emph{NOTE: }ISO recommends that capitalization follow the accepted practice for the language or script in which the information is given.}\\
% See \cite{b20}.

% \item \emph{Basic format for patents (when available online):}\\
% Name of the invention, by inventor's name. (year, month day). Patent Number [Type of medium]. Available: site/path/file\\
% See \cite{b21}.

% \item \emph{Basic format}\emph{for conference proceedings (published):}\\
% J. K. Author, ``Title of paper,'' in \emph{Abbreviated Name of Conf.}, City of Conf., Abbrev. State (if given), Country, year, pp. \emph{xxxxxx.}\\
% See \cite{b22}.

% \item \emph{Example for papers presented at conferences (unpublished):}\\
% See \cite{b23}.

% \item \emph{Basic format for patents}$:$\\
% J. K. Author, ``Title of patent,'' U.S. Patent \emph{x xxx xxx}, Abbrev. Month, day, year.\\
% See \cite{b24}.

% \item \emph{Basic format for theses (M.S.) and dissertations (Ph.D.):}
% \begin{enumerate}
% \item J. K. Author, ``Title of thesis,'' M.S. thesis, Abbrev. Dept., Abbrev. Univ., City of Univ., Abbrev. State, year.
% \item J. K. Author, ``Title of dissertation,'' Ph.D. dissertation, Abbrev. Dept., Abbrev. Univ., City of Univ., Abbrev. State, year.
% \end{enumerate}
% See \cite{b25,b26}.

% \item \emph{Basic format for the most common types of unpublished references:}
% \begin{enumerate}
% \item J. K. Author, private communication, Abbrev. Month, year.
% \item J. K. Author, ``Title of paper,'' unpublished.
% \item J. K. Author, ``Title of paper,'' to be published.
% \end{enumerate}
% See \cite{b27}--\cite{b29}.

% \item \emph{Basic formats for standards:}
% \begin{enumerate}
% \item \emph{Title of Standard}, Standard number, date.
% \item \emph{Title of Standard}, Standard number, Corporate author, location, date.
% \end{enumerate}
% See \cite{b30,b31}.

% \item \emph{Article number in~reference examples:}\\
% See \cite{b32,b33}.

% \item \emph{Example when using et al.:}\\
% See \cite{b34}.

% \end{itemize}

% \begin{thebibliography}{bibl.bib}

% \bibitem{b1} G. O. Young, ``Synthetic structure of industrial plastics,'' in \emph{Plastics,} 2\textsuperscript{nd} ed., vol. 3, J. Peters, Ed. New York, NY, USA: McGraw-Hill, 1964, pp. 15--64.

% \bibitem{b2} W.-K. Chen, \emph{Linear Networks and Systems.} Belmont, CA, USA: Wadsworth, 1993, pp. 123--135.

% \bibitem{b3} J. U. Duncombe, ``Infrared navigation---Part I: An assessment of feasibility,'' \emph{IEEE Trans. Electron Devices}, vol. ED-11, no. 1, pp. 34--39, Jan. 1959, 10.1109/TED.2016.2628402.

% \bibitem{b4} E. P. Wigner, ``Theory of traveling-wave optical laser,'' \emph{Phys. Rev}., vol. 134, pp. A635--A646, Dec. 1965.

% \bibitem{b5} E. H. Miller, ``A note on reflector arrays,'' \emph{IEEE Trans. Antennas Propagat}., to be published.

% \bibitem{b6} E. E. Reber, R. L. Michell, and C. J. Carter, ``Oxygen absorption in the earth's atmosphere,'' Aerospace Corp., Los Angeles, CA, USA, Tech. Rep. TR-0200 (4230-46)-3, Nov. 1988.

% \bibitem{b7} J. H. Davis and J. R. Cogdell, ``Calibration program for the 16-foot antenna,'' Elect. Eng. Res. Lab., Univ. Texas, Austin, TX, USA, Tech. Memo. NGL-006-69-3, Nov. 15, 1987.

% \bibitem{b8} \emph{Transmission Systems for Communications}, 3\textsuperscript{rd} ed., Western Electric Co., Winston-Salem, NC, USA, 1985, pp. 44--60.

% \bibitem{b9} \emph{Motorola Semiconductor Data Manual}, Motorola Semiconductor Products Inc., Phoenix, AZ, USA, 1989.

% \bibitem{b10} G. O. Young, ``Synthetic structure of industrial
% plastics,'' in Plastics, vol. 3, Polymers of Hexadromicon, J. Peters,
% Ed., 2\textsuperscript{nd} ed. New York, NY, USA: McGraw-Hill, 1964, pp. 15-64.
% [Online]. Available:
% \underline{http://www.bookref.com}.

% \bibitem{b11} \emph{The Founders' Constitution}, Philip B. Kurland
% and Ralph Lerner, eds., Chicago, IL, USA: Univ. Chicago Press, 1987.
% [Online]. Available: \underline{http://press-pubs.uchicago.edu/founders/}

% \bibitem{b12} The Terahertz Wave eBook. ZOmega Terahertz Corp., 2014.
% [Online]. Available:
% \underline{http://dl.z-thz.com/eBook/zomega\_ebook\_pdf\_1206\_sr.pdf}. Accessed on: May 19, 2014.

% \bibitem{b13} Philip B. Kurland and Ralph Lerner, eds., \emph{The
% Founders' Constitution.} Chicago, IL, USA: Univ. of Chicago Press,
% 1987, Accessed on: Feb. 28, 2010, [Online] Available:
% \underline{http://press-pubs.uchicago.edu/founders/}

% \bibitem{b14} J. S. Turner, ``New directions in communications,'' \emph{IEEE J. Sel. Areas Commun}., vol. 13, no. 1, pp. 11-23, Jan. 1995.

% \bibitem{b15} W. P. Risk, G. S. Kino, and H. J. Shaw, ``Fiber-optic frequency shifter using a surface acoustic wave incident at an oblique angle,'' \emph{Opt. Lett.}, vol. 11, no. 2, pp. 115--117, Feb. 1986.

% \bibitem{b16} P. Kopyt \emph{et al., ``}Electric properties of graphene-based conductive layers from DC up to terahertz range,'' \emph{IEEE THz Sci. Technol.,} to be published. DOI: 10.1109/TTHZ.2016.2544142.

% \bibitem{b17} PROCESS Corporation, Boston, MA, USA. Intranets:
% Internet technologies deployed behind the firewall for corporate
% productivity. Presented at INET96 Annual Meeting. [Online].
% Available: \underline{http://home.process.com/Intranets/wp2.htp}

% \bibitem{b18} R. J. Hijmans and J. van Etten, ``Raster: Geographic analysis and modeling with raster data,'' R Package Version 2.0-12, Jan. 12, 2012. [Online]. Available: \underline {http://CRAN.R-project.org/package=raster} 

% \bibitem{b19} Teralyzer. Lytera UG, Kirchhain, Germany [Online].
% Available:
% \underline{http://www.lytera.de/Terahertz\_THz\_Spectroscopy.php?id=home}, Accessed on: Jun. 5, 2014

% \bibitem{b20} U.S. House. 102\textsuperscript{nd} Congress, 1\textsuperscript{st} Session. (1991, Jan. 11). \emph{H. Con. Res. 1, Sense of the Congress on Approval of}  \emph{Military Action}. [Online]. Available: LEXIS Library: GENFED File: BILLS

% \bibitem{b21} Musical toothbrush with mirror, by L.M.R. Brooks. (1992, May 19). Patent D 326 189 [Online]. Available: NEXIS Library: LEXPAT File: DES

% \bibitem{b22} D. B. Payne and J. R. Stern, ``Wavelength-switched pas- sively coupled single-mode optical network,'' in \emph{Proc. IOOC-ECOC,} Boston, MA, USA, 1985, pp. 585--590.

% \bibitem{b23} D. Ebehard and E. Voges, ``Digital single sideband detection for interferometric sensors,'' presented at the \emph{2\textsuperscript{nd} Int. Conf. Optical Fiber Sensors,} Stuttgart, Germany, Jan. 2-5, 1984.

% \bibitem{b24} G. Brandli and M. Dick, ``Alternating current fed power supply,'' U.S. Patent 4 084 217, Nov. 4, 1978.

% \bibitem{b25} J. O. Williams, ``Narrow-band analyzer,'' Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, USA, 1993.

% \bibitem{b26} N. Kawasaki, ``Parametric study of thermal and chemical nonequilibrium nozzle flow,'' M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.

% \bibitem{b27} A. Harrison, private communication, May 1995.

% \bibitem{b28} B. Smith, ``An approach to graphs of linear forms,'' unpublished.

% \bibitem{b29} A. Brahms, ``Representation error for real numbers in binary computer arithmetic,'' IEEE Computer Group Repository, Paper R-67-85.

% \bibitem{b30} IEEE Criteria for Class IE Electric Systems, IEEE Standard 308, 1969.

% \bibitem{b31} Letter Symbols for Quantities, ANSI Standard Y10.5-1968.

% \bibitem{b32} R. Fardel, M. Nagel, F. Nuesch, T. Lippert, and A. Wokaun, ``Fabrication of organic light emitting diode pixels by laser-assisted forward transfer,'' \emph{Appl. Phys. Lett.}, vol. 91, no. 6, Aug. 2007, Art. no. 061103.~

% \bibitem{b33} J. Zhang and N. Tansu, ``Optical gain and laser characteristics of InGaN quantum wells on ternary InGaN substrates,'' \emph{IEEE Photon. J.}, vol. 5, no. 2, Apr. 2013, Art. no. 2600111

% \bibitem{b34} S. Azodolmolky~\emph{et al.}, Experimental demonstration of an impairment aware network planning and operation tool for transparent/translucent optical networks,''~\emph{J. Lightw. Technol.}, vol. 29, no. 4, pp. 439--448, Sep. 2011.
% \end{thebibliography}

==> ieeeaccess_suggestions.tex <==
% These instructions give you guidelines for preparing papers for 
% IEEE Access. Use this document as a template if you are 
% using \LaTeX. Otherwise, use this document as an 
% instruction set. The electronic file of your paper will be formatted further 
% at IEEE. Paper titles should be written in uppercase and lowercase letters, 
% not all uppercase. Avoid writing long formulas with subscripts in the title; 
% short formulas that identify the elements are fine (e.g., "Nd--Fe--B"). Do 
% not write ``(Invited)'' in the title. Full names of authors are preferred in 
% the author field, but are not required. Put a space between authors' 
% initials. The abstract must be a concise yet comprehensive reflection of 
% what is in your article. In particular, the abstract must be self-contained, 
% without abbreviations, footnotes, or references. It should be a microcosm of 
% the full article. The abstract must be between 150--250 words. Be sure that 
% you adhere to these limits; otherwise, you will need to edit your abstract 
% accordingly. The abstract must be written as one paragraph, and should not 
% contain displayed mathematical equations or tabular material. The abstract 
% should include three or four different keywords or phrases, as this will 
% help readers to find it. It is important to avoid over-repetition of such 
% phrases as this can result in a page being rejected by search engines. 
% Ensure that your abstract reads well and is grammatically correct.

% Enter key words or phrases in alphabetical 
% order, separated by commas. For a list of suggested keywords, send a blank 
% e-mail to keywords@ieee.org or visit \underline
% {http://www.ieee.org/organizations/pubs/ani\_prod/keywrd98.txt}

% Use one space after periods and colons. Hyphenate complex modifiers: 
% ``zero-field-cooled magnetization.'' Avoid dangling participles, such as, 
% ``Using \eqref{eq}, the potential was calculated.'' [It is not clear who or what 
% used \eqref{eq}.] Write instead, ``The potential was calculated by using \eqref{eq},'' or 
% ``Using \eqref{eq}, we calculated the potential.''

% Use a zero before decimal points: ``0.25,'' not ``.25.'' Use 
% ``cm$^{3}$,'' not ``cc.'' Indicate sample dimensions as ``0.1 cm 
% $\times $ 0.2 cm,'' not ``0.1 $\times $ 0.2 cm$^{2}$.'' The 
% abbreviation for ``seconds'' is ``s,'' not ``sec.'' Use 
% ``Wb/m$^{2}$'' or ``webers per square meter,'' not 
% ``webers/m$^{2}$.'' When expressing a range of values, write ``7 to 
% 9'' or ``7--9,'' not ``7$\sim $9.''

% A parenthetical statement at the end of a sentence is punctuated outside of 
% the closing parenthesis (like this). (A parenthetical sentence is punctuated 
% within the parentheses.) In American English, periods and commas are within 
% quotation marks, like ``this period.'' Other punctuation is ``outside''! 
% Avoid contractions; for example, write ``do not'' instead of ``don't.'' The 
% serial comma is preferred: ``A, B, and C'' instead of ``A, B and C.''

% If you wish, you may write in the first person singular or plural and use 
% the active voice (``I observed that $\ldots$'' or ``We observed that $\ldots$'' 
% instead of ``It was observed that $\ldots$''). Remember to check spelling. If 
% your native language is not English, please get a native English-speaking 
% colleague to carefully proofread your paper.

% Try not to use too many typefaces in the same article. You're writing
% scholarly papers, not ransom notes. Also please remember that MathJax
% can't handle really weird typefaces.

% Number equations consecutively with equation numbers in parentheses flush 
% with the right margin, as in \eqref{eq}. To make your equations more 
% compact, you may use the solidus (~/~), the exp function, or appropriate 
% exponents. Use parentheses to avoid ambiguities in denominators. Punctuate 
% equations when they are part of a sentence, as in
% \begin{equation}E=mc^2.\label{eq}\end{equation}

% Be sure that the symbols in your equation have been defined before the 
% equation appears or immediately following. Italicize symbols ($T$ might refer 
% to temperature, but T is the unit tesla). Refer to ``\eqref{eq},'' not ``Eq. \eqref{eq}'' 
% or ``equation \eqref{eq},'' except at the beginning of a sentence: ``Equation \eqref{eq} 
% is $\ldots$ .''

% Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
% of ``hard'' references (e.g., \verb|(1)|). That will make it possible
% to combine sections, add equations, or change the order of figures or
% citations without having to go through the file line by line.

% Please don't use the \verb|{eqnarray}| equation environment. Use
% \verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
% environment leaves unsightly spaces around relation symbols.
% Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
% will not stop equation numbers inside \verb|{array}| (there won't be
% any anyway) and it might stop a wanted equation number in the
% surrounding equation.

% Please note that the \verb|{subequations}| environment in {\LaTeX}
% will increment the main equation counter even when there are no
% equation numbers displayed. If you forget that, you might write an
% article in which the equation numbers skip from (17) to (20), causing
% the copy editors to wonder if you've discovered a new method of
% counting.

% {\BibTeX} does not work by magic. It doesn't get the bibliographic
% data from thin air but from .bib files. If you use {\BibTeX} to produce a
% bibliography you must send the .bib files. 

% {\LaTeX} can't read your mind. If you assign the same label to a
% subsubsection and a table, you might find that Table I has been cross
% referenced as Table IV-B3. 

% {\LaTeX} does not have precognitive abilities. If you put a
% \verb|\label| command before the command that updates the counter it's
% supposed to be using, the label will pick up the last counter to be
% cross referenced instead. In particular, a \verb|\label| command
% should not go before the caption of a figure or a table.

% Use either SI (MKS) or CGS as primary units. (SI units are strongly 
% encouraged.) English units may be used as secondary units (in parentheses). 
% This applies to papers in data storage. For example, write ``15 
% Gb/cm$^{2}$ (100 Gb/in$^{2})$.'' An exception is when 
% English units are used as identifiers in trade, such as ``3\textonehalf-in 
% disk drive.'' Avoid combining SI and CGS units, such as current in amperes 
% and magnetic field in oersteds. This often leads to confusion because 
% equations do not balance dimensionally. If you must use mixed units, clearly 
% state the units for each quantity in an equation.

% The SI unit for magnetic field strength $H$ is A/m. However, if you wish to use 
% units of T, either refer to magnetic flux density $B$ or magnetic field 
% strength symbolized as $\mu _{0}H$. Use the center dot to separate 
% compound units, e.g., ``A$\cdot $m$^{2}$.''

% The word ``data'' is plural, not singular. The subscript for the 
% permeability of vacuum $\mu _{0}$ is zero, not a lowercase letter 
% ``o.'' The term for residual magnetization is ``remanence''; the adjective 
% is ``remanent''; do not write ``remnance'' or ``remnant.'' Use the word 
% ``micrometer'' instead of ``micron.'' A graph within a graph is an 
% ``inset,'' not an ``insert.'' The word ``alternatively'' is preferred to the 
% word ``alternately'' (unless you really mean something that alternates). Use 
% the word ``whereas'' instead of ``while'' (unless you are referring to 
% simultaneous events). Do not use the word ``essentially'' to mean 
% ``approximately'' or ``effectively.'' Do not use the word ``issue'' as a 
% euphemism for ``problem.'' When compositions are not specified, separate 
% chemical symbols by en-dashes; for example, ``NiMn'' indicates the 
% intermetallic compound Ni$_{0.5}$Mn$_{0.5}$ whereas 
% ``Ni--Mn'' indicates an alloy of some composition 
% Ni$_{x}$Mn$_{1-x}$.

% \Figure[t!](topskip=0pt, botskip=0pt, midskip=0pt)[width=3.25in]{figures/scenario.png}
% {Caption. \label{fig:scenario}}

% Be aware of the different meanings of the homophones ``affect'' (usually a 
% verb) and ``effect'' (usually a noun), ``complement'' and ``compliment,'' 
% ``discreet'' and ``discrete,'' ``principal'' (e.g., ``principal 
% investigator'') and ``principle'' (e.g., ``principle of measurement''). Do 
% not confuse ``imply'' and ``infer.'' 

% Prefixes such as ``non,'' ``sub,'' ``micro,'' ``multi,'' and ``ultra'' are 
% not independent words; they should be joined to the words they modify, 
% usually without a hyphen. There is no period after the ``et'' in the Latin 
% abbreviation ``\emph{et al.}'' (it is also italicized). The abbreviation ``i.e.,'' means 
% ``that is,'' and the abbreviation ``e.g.,'' means ``for example'' (these 
% abbreviations are not italicized).

% A general IEEE styleguide is available at \underline{http://www.ieee.org/}\break\underline{authortools}.

% \subsection{Types of Graphics}
% The following list outlines the different types of graphics published in 
% IEEE journals. They are categorized based on their construction, and use of 
% color/shades of gray:

% \subsubsection{Color/Grayscale figures}
% {Figures that are meant to appear in color, or shades of black/gray. Such 
% figures may include photographs, illustrations, multicolor graphs, and 
% flowcharts.}

% \subsubsection{Line Art figures}
% {Figures that are composed of only black lines and shapes. These figures 
% should have no shades or half-tones of gray, only black and white.}

% \subsubsection{Author photos}
% {Head and shoulders shots of authors that appear at the end of our papers. }

% \subsubsection{Tables}
% {Data charts which are typically black and white, but sometimes include 
% color.}

% \begin{table}
% \caption{Units for Magnetic Properties}
% \label{table}
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{|p{25pt}|p{75pt}|p{115pt}|}
% \hline
% Symbol& 
% Quantity& 
% Conversion from Gaussian and \par CGS EMU to SI $^{\mathrm{a}}$ \\
% \hline
% $\Phi $& 
% magnetic flux& 
% 1 Mx $\to  10^{-8}$ Wb $= 10^{-8}$ V$\cdot $s \\
% $B$& 
% magnetic flux density, \par magnetic induction& 
% 1 G $\to  10^{-4}$ T $= 10^{-4}$ Wb/m$^{2}$ \\
% $H$& 
% magnetic field strength& 
% 1 Oe $\to  10^{3}/(4\pi )$ A/m \\
% $m$& 
% magnetic moment& 
% 1 erg/G $=$ 1 emu \par $\to 10^{-3}$ A$\cdot $m$^{2} = 10^{-3}$ J/T \\
% $M$& 
% magnetization& 
% 1 erg/(G$\cdot $cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 10^{3}$ A/m \\
% 4$\pi M$& 
% magnetization& 
% 1 G $\to  10^{3}/(4\pi )$ A/m \\
% $\sigma $& 
% specific magnetization& 
% 1 erg/(G$\cdot $g) $=$ 1 emu/g $\to $ 1 A$\cdot $m$^{2}$/kg \\
% $j$& 
% magnetic dipole \par moment& 
% 1 erg/G $=$ 1 emu \par $\to 4\pi \times  10^{-10}$ Wb$\cdot $m \\
% $J$& 
% magnetic polarization& 
% 1 erg/(G$\cdot $cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 4\pi \times  10^{-4}$ T \\
% $\chi , \kappa $& 
% susceptibility& 
% 1 $\to  4\pi $ \\
% $\chi_{\rho }$& 
% mass susceptibility& 
% 1 cm$^{3}$/g $\to  4\pi \times  10^{-3}$ m$^{3}$/kg \\
% $\mu $& 
% permeability& 
% 1 $\to  4\pi \times  10^{-7}$ H/m \par $= 4\pi \times  10^{-7}$ Wb/(A$\cdot $m) \\
% $\mu_{r}$& 
% relative permeability& 
% $\mu \to \mu_{r}$ \\
% $w, W$& 
% energy density& 
% 1 erg/cm$^{3} \to  10^{-1}$ J/m$^{3}$ \\
% $N, D$& 
% demagnetizing factor& 
% 1 $\to  1/(4\pi )$ \\
% \hline
% \multicolumn{3}{p{251pt}}{Vertical lines are optional in tables. Statements that serve as captions for 
% the entire table do not need footnote letters. }\\
% \multicolumn{3}{p{251pt}}{$^{\mathrm{a}}$Gaussian units are the same as cg emu for magnetostatics; Mx 
% $=$ maxwell, G $=$ gauss, Oe $=$ oersted; Wb $=$ weber, V $=$ volt, s $=$ 
% second, T $=$ tesla, m $=$ meter, A $=$ ampere, J $=$ joule, kg $=$ 
% kilogram, H $=$ henry.}
% \end{tabular}
% \label{tab1}
% \end{table}

% \subsection{Multipart figures}
% Figures compiled of more than one sub-figure presented side-by-side, or 
% stacked. If a multipart figure is made up of multiple figure
% types (one part is lineart, and another is grayscale or color) the figure 
% should meet the stricter guidelines.

% \subsection{File Formats For Graphics}\label{formats}
% Format and save your graphics using a suitable graphics processing program 
% that will allow you to create the images as PostScript (PS), Encapsulated 
% PostScript (.EPS), Tagged Image File Format (.TIFF), Portable Document 
% Format (.PDF), Portable Network Graphics (.PNG), or Metapost (.MPS), sizes them, and adjusts 
% the resolution settings. When 
% submitting your final paper, your graphics should all be submitted 
% individually in one of these formats along with the manuscript.

% \subsection{Sizing of Graphics}
% Most charts, graphs, and tables are one column wide (3.5 inches/88 
% millimeters/21 picas) or page wide (7.16 inches/181 millimeters/43 
% picas). The maximum depth a graphic can be is 8.5 inches (216 millimeters/54
% picas). When choosing the depth of a graphic, please allow space for a 
% caption. Figures can be sized between column and page widths if the author 
% chooses, however it is recommended that figures are not sized less than 
% column width unless when necessary. 

% There is currently one publication with column measurements that do not 
% coincide with those listed above. Proceedings of the IEEE has a column 
% measurement of 3.25 inches (82.5 millimeters/19.5 picas). 

% The final printed size of author photographs is exactly
% 1 inch wide by 1.25 inches tall (25.4 millimeters$\,\times\,$31.75 millimeters/6 
% picas$\,\times\,$7.5 picas). Author photos printed in editorials measure 1.59 inches 
% wide by 2 inches tall (40 millimeters$\,\times\,$50 millimeters/9.5 picas$\,\times\,$12 
% picas).

% \subsection{Resolution }
% The proper resolution of your figures will depend on the type of figure it 
% is as defined in the ``Types of Figures'' section. Author photographs, 
% color, and grayscale figures should be at least 300dpi. Line art, including 
% tables should be a minimum of 600dpi.

% \subsection{Vector Art}
% In order to preserve the figures' integrity across multiple computer 
% platforms, we accept files in the following formats: .EPS/.PDF/.PS. All 
% fonts must be embedded or text converted to outlines in order to achieve the 
% best-quality results.

% \subsection{Color Space}
% The term color space refers to the entire sum of colors that can be 
% represented within the said medium. For our purposes, the three main color 
% spaces are Grayscale, RGB (red/green/blue) and CMYK 
% (cyan/magenta/yellow/black). RGB is generally used with on-screen graphics, 
% whereas CMYK is used for printing purposes.

% All color figures should be generated in RGB or CMYK color space. Grayscale 
% images should be submitted in Grayscale color space. Line art may be 
% provided in grayscale OR bitmap colorspace. Note that ``bitmap colorspace'' 
% and ``bitmap file format'' are not the same thing. When bitmap color space 
% is selected, .TIF/.TIFF/.PNG are the recommended file formats.

% \subsection{Accepted Fonts Within Figures}
% When preparing your graphics IEEE suggests that you use of one of the 
% following Open Type fonts: Times New Roman, Helvetica, Arial, Cambria, and 
% Symbol. If you are supplying EPS, PS, or PDF files all fonts must be 
% embedded. Some fonts may only be native to your operating system; without 
% the fonts embedded, parts of the graphic may be distorted or missing.

% A safe option when finalizing your figures is to strip out the fonts before 
% you save the files, creating ``outline'' type. This converts fonts to 
% artwork what will appear uniformly on any screen.

% \subsection{Using Labels Within Figures}

% \subsubsection{Figure Axis labels }
% Figure axis labels are often a source of confusion. Use words rather than 
% symbols. As an example, write the quantity ``Magnetization,'' or 
% ``Magnetization M,'' not just ``M.'' Put units in parentheses. Do not label 
% axes only with units. As in Fig. 1, for example, write ``Magnetization 
% (A/m)'' or ``Magnetization (A$\cdot$m$^{-1}$),'' not just ``A/m.'' Do not label axes with a ratio of quantities and 
% units. For example, write ``Temperature (K),'' not ``Temperature/K.'' 

% Multipliers can be especially confusing. Write ``Magnetization (kA/m)'' or 
% ``Magnetization (10$^{3}$ A/m).'' Do not write ``Magnetization 
% (A/m)$\,\times\,$1000'' because the reader would not know whether the top 
% axis label in Fig. 1 meant 16000 A/m or 0.016 A/m. Figure labels should be 
% legible, approximately 8 to 10 point type.

% \subsubsection{Subfigure Labels in Multipart Figures and Tables}
% Multipart figures should be combined and labeled before final submission. 
% Labels should appear centered below each subfigure in 8 point Times New 
% Roman font in the format of (a) (b) (c). 

% \subsection{Referencing a Figure or Table Within Your Paper}
% When referencing your figures and tables within your paper, use the 
% abbreviation ``Fig.'' even at the beginning of a sentence. Do not abbreviate 
% ``Table.'' Tables should be numbered with Roman Numerals.

% \subsection{Checking Your Figures: The IEEE Graphics Analyzer}
% The IEEE Graphics Analyzer enables authors to pre-screen their graphics for 
% compliance with IEEE Access standards before submission. 
% The online tool, located at
% \underline{http://graphicsqc.ieee.org/}, allows authors to 
% upload their graphics in order to check that each file is the correct file 
% format, resolution, size and colorspace; that no fonts are missing or 
% corrupt; that figures are not compiled in layers or have transparency, and 
% that they are named according to the IEEE Access naming 
% convention. At the end of this automated process, authors are provided with 
% a detailed report on each graphic within the web applet, as well as by 
% email.

% For more information on using the Graphics Analyzer or any other graphics 
% related topic, contact the IEEE Graphics Help Desk by e-mail at 
% graphics@ieee.org.

% \subsection{Submitting Your Graphics}
% Because IEEE will do the final formatting of your paper,
% you do not need to position figures and tables at the top and bottom of each 
% column. In fact, all figures, figure captions, and tables can be placed at 
% the end of your paper. In addition to, or even in lieu of submitting figures 
% within your final manuscript, figures should be submitted individually, 
% separate from the manuscript in one of the file formats listed above in 
% Section \ref{formats}. Place figure captions below the figures; place table titles 
% above the tables. Please do not include captions as part of the figures, or 
% put them in ``text boxes'' linked to the figures. Also, do not place borders 
% around the outside of your figures.

% \subsection{Color Processing/Printing in IEEE Journals}
% All IEEE Transactions, Journals, and Letters allow an author to publish 
% color figures on IEEE Xplore\textregistered\ at no charge, and automatically 
% convert them to grayscale for print versions. In most journals, figures and 
% tables may alternatively be printed in color if an author chooses to do so. 
% Please note that this service comes at an extra expense to the author. If 
% you intend to have print color graphics, include a note with your final 
% paper indicating which figures or tables you would like to be handled that 
% way, and stating that you are willing to pay the additional fee.

% A conclusion section is not required. Although a conclusion may review the 
% main points of the paper, do not replicate the abstract as the conclusion. A 
% conclusion might elaborate on the importance of the work or suggest 
% applications and extensions. 

% Appendixes, if needed, appear before the acknowledgment.

% \section*{Acknowledgment}

% The preferred spelling of the word ``acknowledgment'' in American English is 
% without an ``e'' after the ``g.'' Use the singular heading even if you have 
% many acknowledgments. Avoid expressions such as ``One of us (S.B.A.) would 
% like to thank $\ldots$ .'' Instead, write ``F. A. Author thanks $\ldots$ .'' In most 
% cases, sponsor and financial support acknowledgments are placed in the 
% unnumbered footnote on the first page, not here.

% \section*{References and Footnotes}

% \subsection{References}
% References need not be cited in text. When they are, they appear on the 
% line, in square brackets, inside the punctuation. Multiple references are 
% each numbered with separate brackets. When citing a section in a book, 
% please give the relevant page numbers. In text, refer simply to the 
% reference number. Do not use ``Ref.'' or ``reference'' except at the 
% beginning of a sentence: ``Reference b3 shows $\ldots$ .'' Please do not use 
% automatic endnotes in \emph{Word}, rather, type the reference list at the end of the 
% paper using the ``References'' style. \GC{Added a trial reference \cite{3gpp22874}}.

% Reference numbers are set flush left and form a column of their own, hanging 
% out beyond the body of the reference. The reference numbers are on the line, 
% enclosed in square brackets. In all references, the given name of the author 
% or editor is abbreviated to the initial only and precedes the last name. Use 
% them all; use \emph{et al.} only if names are not given. Use commas around Jr., 
% Sr., and III in names. Abbreviate conference titles. When citing IEEE 
% transactions, provide the issue number, page range, volume number, year, 
% and/or month if available. When referencing a patent, provide the day and 
% the month of issue, or application. References may not include all 
% information; please obtain and include relevant information. Do not combine 
% references. There must be only one reference with each number. If there is a 
% URL included with the print reference, it can be included at the end of the 
% reference. 

% Other than books, capitalize only the first word in a paper title, except 
% for proper nouns and element symbols. For papers published in translation 
% journals, please give the English citation first, followed by the original 
% foreign-language citation See the end of this document for formats and 
% examples of common references. For a complete discussion of references and 
% their formats, see the IEEE style manual at
% \underline{http://www.ieee.org/authortools}.


% \section{Submitting Your Paper for Review}

% \subsection{Final Stage}
% When you submit your final version (after your paper has been accepted), 
% print it in two-column format, including figures and tables. You must also 
% send your final manuscript on a disk, via e-mail, or through a Web 
% manuscript submission system as directed by the society contact. You may use 
% \emph{Zip} for large files, or compress files using \emph{Compress, Pkzip, Stuffit,} or \emph{Gzip.} 

% Also, send a sheet of paper or PDF with complete contact information for all 
% authors. Include full mailing addresses, telephone numbers, fax numbers, and 
% e-mail addresses. This information will be used to send each author a 
% complimentary copy of the journal in which the paper appears. In addition, 
% designate one author as the ``corresponding author.'' This is the author to 
% whom proofs of the paper will be sent. Proofs are sent to the corresponding 
% author only.

% \subsection{Review Stage Using ScholarOne\textregistered\ Manuscripts}
% Contributions to the Transactions, Journals, and Letters may be submitted 
% electronically on IEEE's on-line manuscript submission and peer-review 
% system, ScholarOne\textregistered\ Manuscripts. You can get a listing of the 
% publications that participate in ScholarOne at 
% \underline{http://www.ieee.org/publications\_standards/publications/}\break\underline{authors/authors\_submission.html}.
% First check if you have an existing account. If there is none, please create 
% a new account. After logging in, go to your Author Center and click ``Submit 
% First Draft of a New Manuscript.'' 

% Along with other information, you will be asked to select the subject from a 
% pull-down list. Depending on the journal, there are various steps to the 
% submission process; you must complete all steps for a complete submission. 
% At the end of each step you must click ``Save and Continue''; just uploading 
% the paper is not sufficient. After the last step, you should see a 
% confirmation that the submission is complete. You should also receive an 
% e-mail confirmation. For inquiries regarding the submission of your paper on 
% ScholarOne Manuscripts, please contact oprs-support@ieee.org or call +1 732 
% 465 5861.

% ScholarOne Manuscripts will accept files for review in various formats. 
% Please check the guidelines of the specific journal for which you plan to 
% submit.

% You will be asked to file an electronic copyright form immediately upon 
% completing the submission process (authors are responsible for obtaining any 
% security clearances). Failure to submit the electronic copyright could 
% result in publishing delays later. You will also have the opportunity to 
% designate your article as ``open access'' if you agree to pay the IEEE open 
% access fee. 

% \subsection{Final Stage Using ScholarOne Manuscripts}
% Upon acceptance, you will receive an email with specific instructions 
% regarding the submission of your final files. To avoid any delays in 
% publication, please be sure to follow these instructions. Most journals 
% require that final submissions be uploaded through ScholarOne Manuscripts, 
% although some may still accept final submissions via email. Final 
% submissions should include source files of your accepted manuscript, high 
% quality graphic files, and a formatted pdf file. If you have any questions 
% regarding the final submission process, please contact the administrative 
% contact for the journal. 

% In addition to this, upload a file with complete contact information for all 
% authors. Include full mailing addresses, telephone numbers, fax numbers, and 
% e-mail addresses. Designate the author who submitted the manuscript on 
% ScholarOne Manuscripts as the ``corresponding author.'' This is the only 
% author to whom proofs of the paper will be sent. 

% \subsection{Footnotes}
% Number footnotes separately in superscript numbers.\footnote{It is recommended that footnotes be avoided (except for 
% the unnumbered footnote with the receipt date on the first page). Instead, 
% try to integrate the footnote information into the text.} Place the actual 
% footnote at the bottom of the column in which it is cited; do not put 
% footnotes in the reference list (endnotes). Use letters for table footnotes 
% (see Table \ref{table}).

% \subsection{Copyright Form}
% Authors must submit an electronic IEEE Copyright Form (eCF) upon submitting 
% their final manuscript files. You can access the eCF system through your 
% manuscript submission system or through the Author Gateway. You are 
% responsible for obtaining any necessary approvals and/or security 
% clearances. For additional information on intellectual property rights, 
% visit the IEEE Intellectual Property Rights department web page at 
% \underline{http://www.ieee.org/publications\_standards/publications/}\break\underline{rights/index.html}. 

% \section{IEEE Publishing Policy}
% The general IEEE policy requires that authors should only submit original 
% work that has neither appeared elsewhere for publication, nor is under 
% review for another refereed publication. The submitting author must disclose 
% all prior publication(s) and current submissions when submitting a 
% manuscript. Do not publish ``preliminary'' data or results. The submitting 
% author is responsible for obtaining agreement of all coauthors and any 
% consent required from employers or sponsors before submitting an article. 
% The IEEE Access Department strongly discourages courtesy 
% authorship; it is the obligation of the authors to cite only relevant prior 
% work.

% The IEEE Access Department does not publish conference 
% records or proceedings, but can publish articles related to conferences that 
% have undergone rigorous peer review. Minimally, two reviews are required for 
% every article submitted for peer review.

% \section{Publication Principles}
% The two types of contents of that are published are; 1) peer-reviewed and 2) 
% archival. The Access Department publishes scholarly 
% articles of archival value as well as tutorial expositions and critical 
% reviews of classical subjects and topics of current interest. 

% Authors should consider the following points:

% \begin{enumerate}
% \item Technical papers submitted for publication must advance the state of knowledge and must cite relevant prior work. 
% \item The length of a submitted paper should be commensurate with the importance, or appropriate to the complexity, of the work. For example, an obvious extension of previously published work might not be appropriate for publication or might be adequately treated in just a few pages.
% \item Authors must convince both peer reviewers and the editors of the scientific and technical merit of a paper; the standards of proof are higher when extraordinary or unexpected results are reported. 
% \item Because replication is required for scientific progress, papers submitted for publication must provide sufficient information to allow readers to perform similar experiments or calculations and 
% use the reported results. Although not everything need be disclosed, a paper 
% must contain new, useable, and fully described information. For example, a 
% specimen's chemical composition need not be reported if the main purpose of 
% a paper is to introduce a new measurement technique. Authors should expect 
% to be challenged by reviewers if the results are not supported by adequate 
% data and critical details.
% \item Papers that describe ongoing work or announce the latest technical achievement, which are suitable for presentation at a professional conference, may not be appropriate for publication.
% \end{enumerate}

% \section{Reference Examples}

% \begin{itemize}

% \item \emph{Basic format for books:}\\
% J. K. Author, ``Title of chapter in the book,'' in \emph{Title of His Published Book, x}th ed. City of Publisher, (only U.S. State), Country: Abbrev. of Publisher, year, ch. $x$, sec. $x$, pp. \emph{xxx--xxx.}\\
% See \cite{b1,b2}.

% \item \emph{Basic format for periodicals:}\\
% J. K. Author, ``Name of paper,'' \emph{Abbrev. Title of Periodical}, vol. \emph{x, no}. $x, $pp\emph{. xxx--xxx, }Abbrev. Month, year, DOI. 10.1109.\emph{XXX}.123456.\\
% See \cite{b3}--\cite{b5}.

% \item \emph{Basic format for reports:}\\
% J. K. Author, ``Title of report,'' Abbrev. Name of Co., City of Co., Abbrev. State, Country, Rep. \emph{xxx}, year.\\
% See \cite{b6,b7}.

% \item \emph{Basic format for handbooks:}\\
% \emph{Name of Manual/Handbook, x} ed., Abbrev. Name of Co., City of Co., Abbrev. State, Country, year, pp. \emph{xxx--xxx.}\\
% See \cite{b8,b9}.

% \item \emph{Basic format for books (when available online):}\\
% J. K. Author, ``Title of chapter in the book,'' in \emph{Title of
% Published Book}, $x$th ed. City of Publisher, State, Country: Abbrev.
% of Publisher, year, ch. $x$, sec. $x$, pp. \emph{xxx--xxx}. [Online].
% Available: \underline{http://www.web.com}\\
% See \cite{b10}--\cite{b13}.

% \item \emph{Basic format for journals (when available online):}\\
% J. K. Author, ``Name of paper,'' \emph{Abbrev. Title of Periodical}, vol. $x$, no. $x$, pp. \emph{xxx--xxx}, Abbrev. Month, year. Accessed on: Month, Day, year, DOI: 10.1109.\emph{XXX}.123456, [Online].\\
% See \cite{b14}--\cite{b16}.

% \item \emph{Basic format for papers presented at conferences (when available online): }\\
% J.K. Author. (year, month). Title. presented at abbrev. conference title. [Type of Medium]. Available: site/path/file\\
% See \cite{b17}.

% \item \emph{Basic format for reports and handbooks (when available online):}\\
% J. K. Author. ``Title of report,'' Company. City, State, Country. Rep. no., (optional: vol./issue), Date. [Online] Available: site/path/file\\
% See \cite{b18,b19}.

% \item \emph{Basic format for computer programs and electronic documents (when available online): }\\
% Legislative body. Number of Congress, Session. (year, month day). \emph{Number of bill or resolution}, \emph{Title}. [Type of medium]. Available: site/path/file\\
% \textbf{\emph{NOTE: }ISO recommends that capitalization follow the accepted practice for the language or script in which the information is given.}\\
% See \cite{b20}.

% \item \emph{Basic format for patents (when available online):}\\
% Name of the invention, by inventor's name. (year, month day). Patent Number [Type of medium]. Available: site/path/file\\
% See \cite{b21}.

% \item \emph{Basic format}\emph{for conference proceedings (published):}\\
% J. K. Author, ``Title of paper,'' in \emph{Abbreviated Name of Conf.}, City of Conf., Abbrev. State (if given), Country, year, pp. \emph{xxxxxx.}\\
% See \cite{b22}.

% \item \emph{Example for papers presented at conferences (unpublished):}\\
% See \cite{b23}.

% \item \emph{Basic format for patents}$:$\\
% J. K. Author, ``Title of patent,'' U.S. Patent \emph{x xxx xxx}, Abbrev. Month, day, year.\\
% See \cite{b24}.

% \item \emph{Basic format for theses (M.S.) and dissertations (Ph.D.):}
% \begin{enumerate}
% \item J. K. Author, ``Title of thesis,'' M.S. thesis, Abbrev. Dept., Abbrev. Univ., City of Univ., Abbrev. State, year.
% \item J. K. Author, ``Title of dissertation,'' Ph.D. dissertation, Abbrev. Dept., Abbrev. Univ., City of Univ., Abbrev. State, year.
% \end{enumerate}
% See \cite{b25,b26}.

% \item \emph{Basic format for the most common types of unpublished references:}
% \begin{enumerate}
% \item J. K. Author, private communication, Abbrev. Month, year.
% \item J. K. Author, ``Title of paper,'' unpublished.
% \item J. K. Author, ``Title of paper,'' to be published.
% \end{enumerate}
% See \cite{b27}--\cite{b29}.

% \item \emph{Basic formats for standards:}
% \begin{enumerate}
% \item \emph{Title of Standard}, Standard number, date.
% \item \emph{Title of Standard}, Standard number, Corporate author, location, date.
% \end{enumerate}
% See \cite{b30,b31}.

% \item \emph{Article number in~reference examples:}\\
% See \cite{b32,b33}.

% \item \emph{Example when using et al.:}\\
% See \cite{b34}.

% \end{itemize}

% \begin{thebibliography}{bibl.bib}

% \bibitem{b1} G. O. Young, ``Synthetic structure of industrial plastics,'' in \emph{Plastics,} 2\textsuperscript{nd} ed., vol. 3, J. Peters, Ed. New York, NY, USA: McGraw-Hill, 1964, pp. 15--64.

% \bibitem{b2} W.-K. Chen, \emph{Linear Networks and Systems.} Belmont, CA, USA: Wadsworth, 1993, pp. 123--135.

% \bibitem{b3} J. U. Duncombe, ``Infrared navigation---Part I: An assessment of feasibility,'' \emph{IEEE Trans. Electron Devices}, vol. ED-11, no. 1, pp. 34--39, Jan. 1959, 10.1109/TED.2016.2628402.

% \bibitem{b4} E. P. Wigner, ``Theory of traveling-wave optical laser,'' \emph{Phys. Rev}., vol. 134, pp. A635--A646, Dec. 1965.

% \bibitem{b5} E. H. Miller, ``A note on reflector arrays,'' \emph{IEEE Trans. Antennas Propagat}., to be published.

% \bibitem{b6} E. E. Reber, R. L. Michell, and C. J. Carter, ``Oxygen absorption in the earth's atmosphere,'' Aerospace Corp., Los Angeles, CA, USA, Tech. Rep. TR-0200 (4230-46)-3, Nov. 1988.

% \bibitem{b7} J. H. Davis and J. R. Cogdell, ``Calibration program for the 16-foot antenna,'' Elect. Eng. Res. Lab., Univ. Texas, Austin, TX, USA, Tech. Memo. NGL-006-69-3, Nov. 15, 1987.

% \bibitem{b8} \emph{Transmission Systems for Communications}, 3\textsuperscript{rd} ed., Western Electric Co., Winston-Salem, NC, USA, 1985, pp. 44--60.

% \bibitem{b9} \emph{Motorola Semiconductor Data Manual}, Motorola Semiconductor Products Inc., Phoenix, AZ, USA, 1989.

% \bibitem{b10} G. O. Young, ``Synthetic structure of industrial
% plastics,'' in Plastics, vol. 3, Polymers of Hexadromicon, J. Peters,
% Ed., 2\textsuperscript{nd} ed. New York, NY, USA: McGraw-Hill, 1964, pp. 15-64.
% [Online]. Available:
% \underline{http://www.bookref.com}.

% \bibitem{b11} \emph{The Founders' Constitution}, Philip B. Kurland
% and Ralph Lerner, eds., Chicago, IL, USA: Univ. Chicago Press, 1987.
% [Online]. Available: \underline{http://press-pubs.uchicago.edu/founders/}

% \bibitem{b12} The Terahertz Wave eBook. ZOmega Terahertz Corp., 2014.
% [Online]. Available:
% \underline{http://dl.z-thz.com/eBook/zomega\_ebook\_pdf\_1206\_sr.pdf}. Accessed on: May 19, 2014.

% \bibitem{b13} Philip B. Kurland and Ralph Lerner, eds., \emph{The
% Founders' Constitution.} Chicago, IL, USA: Univ. of Chicago Press,
% 1987, Accessed on: Feb. 28, 2010, [Online] Available:
% \underline{http://press-pubs.uchicago.edu/founders/}

% \bibitem{b14} J. S. Turner, ``New directions in communications,'' \emph{IEEE J. Sel. Areas Commun}., vol. 13, no. 1, pp. 11-23, Jan. 1995.

% \bibitem{b15} W. P. Risk, G. S. Kino, and H. J. Shaw, ``Fiber-optic frequency shifter using a surface acoustic wave incident at an oblique angle,'' \emph{Opt. Lett.}, vol. 11, no. 2, pp. 115--117, Feb. 1986.

% \bibitem{b16} P. Kopyt \emph{et al., ``}Electric properties of graphene-based conductive layers from DC up to terahertz range,'' \emph{IEEE THz Sci. Technol.,} to be published. DOI: 10.1109/TTHZ.2016.2544142.

% \bibitem{b17} PROCESS Corporation, Boston, MA, USA. Intranets:
% Internet technologies deployed behind the firewall for corporate
% productivity. Presented at INET96 Annual Meeting. [Online].
% Available: \underline{http://home.process.com/Intranets/wp2.htp}

% \bibitem{b18} R. J. Hijmans and J. van Etten, ``Raster: Geographic analysis and modeling with raster data,'' R Package Version 2.0-12, Jan. 12, 2012. [Online]. Available: \underline {http://CRAN.R-project.org/package=raster} 

% \bibitem{b19} Teralyzer. Lytera UG, Kirchhain, Germany [Online].
% Available:
% \underline{http://www.lytera.de/Terahertz\_THz\_Spectroscopy.php?id=home}, Accessed on: Jun. 5, 2014

% \bibitem{b20} U.S. House. 102\textsuperscript{nd} Congress, 1\textsuperscript{st} Session. (1991, Jan. 11). \emph{H. Con. Res. 1, Sense of the Congress on Approval of}  \emph{Military Action}. [Online]. Available: LEXIS Library: GENFED File: BILLS

% \bibitem{b21} Musical toothbrush with mirror, by L.M.R. Brooks. (1992, May 19). Patent D 326 189 [Online]. Available: NEXIS Library: LEXPAT File: DES

% \bibitem{b22} D. B. Payne and J. R. Stern, ``Wavelength-switched pas- sively coupled single-mode optical network,'' in \emph{Proc. IOOC-ECOC,} Boston, MA, USA, 1985, pp. 585--590.

% \bibitem{b23} D. Ebehard and E. Voges, ``Digital single sideband detection for interferometric sensors,'' presented at the \emph{2\textsuperscript{nd} Int. Conf. Optical Fiber Sensors,} Stuttgart, Germany, Jan. 2-5, 1984.

% \bibitem{b24} G. Brandli and M. Dick, ``Alternating current fed power supply,'' U.S. Patent 4 084 217, Nov. 4, 1978.

% \bibitem{b25} J. O. Williams, ``Narrow-band analyzer,'' Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, USA, 1993.

% \bibitem{b26} N. Kawasaki, ``Parametric study of thermal and chemical nonequilibrium nozzle flow,'' M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.

% \bibitem{b27} A. Harrison, private communication, May 1995.

% \bibitem{b28} B. Smith, ``An approach to graphs of linear forms,'' unpublished.

% \bibitem{b29} A. Brahms, ``Representation error for real numbers in binary computer arithmetic,'' IEEE Computer Group Repository, Paper R-67-85.

% \bibitem{b30} IEEE Criteria for Class IE Electric Systems, IEEE Standard 308, 1969.

% \bibitem{b31} Letter Symbols for Quantities, ANSI Standard Y10.5-1968.

% \bibitem{b32} R. Fardel, M. Nagel, F. Nuesch, T. Lippert, and A. Wokaun, ``Fabrication of organic light emitting diode pixels by laser-assisted forward transfer,'' \emph{Appl. Phys. Lett.}, vol. 91, no. 6, Aug. 2007, Art. no. 061103.~

% \bibitem{b33} J. Zhang and N. Tansu, ``Optical gain and laser characteristics of InGaN quantum wells on ternary InGaN substrates,'' \emph{IEEE Photon. J.}, vol. 5, no. 2, Apr. 2013, Art. no. 2600111

% \bibitem{b34} S. Azodolmolky~\emph{et al.}, Experimental demonstration of an impairment aware network planning and operation tool for transparent/translucent optical networks,''~\emph{J. Lightw. Technol.}, vol. 29, no. 4, pp. 439--448, Sep. 2011.
% \end{thebibliography}
